libcll: an Extendable Python Toolkit for Complementary-Label Learning

Complementary-label learning (CLL) is a weakly supervised learning paradigm for multiclass classification, where only complementary labels -- indicating classes an instance does not belong to -- are provided to the learning algorithm. Despite CLL's increasing popularity, previous studies highlight two main challenges: (1) inconsistent results arising from varied assumptions on complementary label generation, and (2) high barriers to entry due to the lack of a standardized evaluation platform across datasets and algorithms. To address these challenges, we introduce \texttt{libcll}, an extensible Python toolkit for CLL research. \texttt{libcll} provides a universal interface that supports a wide range of generation assumptions, both synthetic and real-world datasets, and key CLL algorithms. The toolkit is designed to mitigate inconsistencies and streamline the research process, with easy installation, comprehensive usage guides, and quickstart tutorials that facilitate efficient adoption and implementation of CLL techniques. Extensive ablation studies conducted with \texttt{libcll} demonstrate its utility in generating valuable insights to advance future CLL research.

==> Figures/fwd-interpolation.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/fwd-int-joint.png}
    \caption{The last epoch accuracy of CLCIFAR10 and CLCIFAR20 for FWD algorithm with an $\alpha$-interpolated transition matrix $T_{\text{int}}$. The five solid points on each cruve represent different noise cleaning rate: 0\%, 25\%, 50\%, 75\%, 100\% from left to right.}
    \label{fig:int}
\end{figure}

==> Figures/label-distribution.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth, valign=t]{Figures/clcifar10_label-distribution.png}
  \includegraphics[width=0.45\textwidth, valign=t]{Figures/clcifar20_label-distribution.png}
  \caption{
  The label distribution of CLCIFAR10 (left) and CLCIFAR20 (right).
  }
  \label{fig:label-dist}
  % \vskip -0.2in
\end{figure}

==> Figures/noise-cleaning.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/data_cleaning_graph/fwd-u-fwd-r-clcifar10.png}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/noise-cleaning-fwd-uniform-cifar10.png}
    \end{subfigure}
    \caption{Accuracy of FWD-U and FWD-R on the noise-removed CLCIFAR10 dataset (\textbf{Left}) and the uniform-CIFAR10 dataset with uniform noise (\textbf{Right}) at varying noise rates.}
    \label{fig:exp-noise}
    % \vskip -0.2in
\end{figure}

==> Figures/overfitting-curve.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/overfitting.png}
    \caption{The Overfitting accuracy curve of FWD, URE, SCL-NL, L-W. The dotted line represents the accuracy obtained without data augmentation, while the solid line represents the accuracy with data augmentation included for reference. The accuracy of FWD, SCL-NL, SCL-EXP, L-W, L-UW methods reaches its highest at approximately the 50 epoches and converges to some lower point. The detail numbers are in appendix~\ref{tab:without-aug}}
    \label{fig:overfit}
\end{figure}

==> Figures/three_trial_label_dist.tex <==
\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{Figures/three_trial_clcifar10.png}
    \caption{CLCIFAR10}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{Figures/three_trial_clcifar20.png}
    \caption{CLCIFAR20}
  \end{subfigure}
  \caption{The complementary label distribution of three independent trials of CLCIFAR10 dataset (\textbf{Left}) and CLCIFAR20 dataset (\textbf{Right}).}
  \label{fig:three_trial_label_dist}
  %\vskip -0.2in
\end{figure}

==> Figures/transition-matrix.tex <==
\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{clcifar10-T.png}
    \caption{CLCIFAR10}
    \label{fig:img1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{clcifar20-T.png}
    \caption{CLCIFAR20}
    \label{fig:img2}
  \end{subfigure}
  \caption{The empirical transition matrices of CLCIFAR10 and CLCIFAR20. The label names of CLCIFAR20 are abbreviated as indexes to save space. The full label names are provided in Appendix~\ref{A:label_names}.}
  \label{fig:twoimgs}
  %\vskip -0.2in
\end{figure}

==> Sections/Checklist.tex <==
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Appendix~\ref{sec:borader-impacts}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Appendix~\ref{sec:link}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{sec:exp_setup}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{sec:exp_setup}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{We cite the all datasets paper as required.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Tables/Biased.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of testing accuracies with different levels of deviation in transition matrices.}
% \vskip 0.15in
\label{tab:biased}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{lccccccccccccccccccc}
\toprule
& \multicolumn{2}{c}{MNIST} & & \multicolumn{2}{c}{KMNIST} & & \multicolumn{2}{c}{FMNIST} & & \multicolumn{2}{c}{CIFAR10} & & \multicolumn{2}{c}{MIN10} & & \multicolumn{2}{c}{Avg.} \\
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12} \cmidrule{14-15} \cmidrule{17-18}
& Weak & Strong & & Weak & Strong & & Weak & Strong & & Weak & Strong & & Weak & Strong & & Weak & Strong \\
\midrule
SCL-NL	&	92.13	&	27.94	&		&	63.07	&	18.13	&		&	82.47	&	26.20	&		&	\bf{62.39}	&	25.89	&		&	\bf{32.33}	&	24.84	&		&	\bf{66.48}	&	24.60\\
SCL-EXP	&	92.01	&	27.53	&		&	63.51	&	15.62	&		&	\bf{82.75}	&	27.38	&		&	61.97	&	27.16	&		&	29.38	&	25.26	&		&	65.92	&	24.59\\
URE-NN	&	91.12	&	27.50	&		&	68.41	&	20.00	&		&	81.03	&	\bf{38.90}	&		&	49.15	&	28.35	&		&	31.35	&	\bf{30.64}	&		&	64.21	&	\bf{29.08}\\
URE-GA	&	\bf{92.55}	&	\bf{38.54}	&		&	\bf{70.43}	&	16.41	&		&	82.13	&	28.91	&		&	61.37	&	26.57	&		&	25.80	&	28.66	&		&	66.46	&	27.82\\
DM	&	90.41	&	29.36	&		&	62.48	&	\bf{23.23}	&		&	81.86	&	32.41	&		&	53.05	&	\bf{29.32}	&		&	31.63	&	21.79	&		&	63.89	&	27.22\\
\midrule
FWD	&	\bf{92.34}	&	\bf{95.71}	&		&	64.38	&	\bf{79.55}	&		&	\bf{83.61}	&	86.22	&		&	59.88	&	74.12	&		&	38.21	&	53.97	&		&	67.68	&	77.91\\
URE-TNN	&	86.21	&	87.68	&		&	59.56	&	65.05	&		&	80.57	&	81.66	&		&	39.54	&	50.41	&		&	30.73	&	25.35	&		&	59.32	&	62.03\\
URE-TGA	&	90.24	&	90.41	&		&	\bf{65.67}	&	68.42	&		&	81.68	&	82.14	&		&	59.82	&	70.00	&		&	34.67	&	44.72	&		&	66.42	&	71.14\\
CPE-I	&	87.64	&	93.19	&		&	61.96	&	73.83	&		&	79.75	&	84.41	&		&	49.00	&	68.61	&		&	26.27	&	45.08	&		&	60.92	&	73.02\\
CPE-F	&	92.24	&	95.67	&		&	64.30	&	79.20	&		&	82.90	&	86.30	&		&	59.80	&	\bf{74.25}	&		&	36.62	&	\bf{54.18}	&		&	67.17	&	\bf{77.92}\\
CPE-T	&	92.18	&	95.57	&		&	63.84	&	78.88	&		&	83.49	&	\bf{86.36}	&		&	\bf{60.38}	&	72.65	&		&	\bf{38.81}	&	53.36	&		&	\bf{67.74}	&	77.36\\
\bottomrule
\end{tabular}%
}
\end{table}

==> Tables/Multi-Hard-New.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of test accuracies where instances have 3 CLs on Real-World datasets.}
% \vskip 0.15in
\label{tab:multi-hard}
% \resizebox{1\linewidth}{!}{%
\scalebox{0.75}{
\begin{tabular}{lcccccccccccccccc}
\toprule
% & \multicolumn{2}{c}{CLCIFAR10} & & \multicolumn{2}{c}{CLCIFAR20} & & \multicolumn{2}{c}{CLMIN10} & & \multicolumn{2}{c}{CLMIN20} & & \multicolumn{2}{c}{Avg.} \\
& {CLCIFAR10} & & {CLCIFAR20} & & {CLMIN10} & & {CLMIN20} & & Avg Rank \\
\midrule
SCL-NL & \bf{47.30\scriptsize{$\pm$0.50}} & & 8.59\scriptsize{$\pm$0.75} & & 12.87\scriptsize{$\pm$2.33} & & 6.87\scriptsize{$\pm$0.39} & & 3.75\\
SCL-EXP & 47.12\scriptsize{$\pm$0.91} & & 9.74\scriptsize{$\pm$0.52} & & 12.78\scriptsize{$\pm$1.42} & & 7.10\scriptsize{$\pm$0.83} & & 3.50\\
URE-NN & 40.74\scriptsize{$\pm$1.12} & & \bf{18.43\scriptsize{$\pm$0.27}} & & \bf{21.78\scriptsize{$\pm$2.66}} & & 7.16\scriptsize{$\pm$0.70} & & 2.75\\
URE-GA & 47.02\scriptsize{$\pm$0.45} & & 14.07\scriptsize{$\pm$0.60} & & 20.83\scriptsize{$\pm$2.88} & & \bf{7.71\scriptsize{$\pm$1.24}} & & \bf{2.00}\\
DM & 46.89\scriptsize{$\pm$0.32} & & 9.11\scriptsize{$\pm$0.31} & & 14.46\scriptsize{$\pm$2.22} & & 6.84\scriptsize{$\pm$0.62} & & 4.50\\
MCL-MAE & 19.83\scriptsize{$\pm$2.91} & & 7.88\scriptsize{$\pm$0.28} & & 11.57\scriptsize{$\pm$0.80} & & 6.64\scriptsize{$\pm$0.89} & & 7.50\\
MCL-EXP & 46.97\scriptsize{$\pm$1.23} & & 8.42\scriptsize{$\pm$0.27} & & 12.37\scriptsize{$\pm$1.61} & & 6.62\scriptsize{$\pm$1.03} & & 6.25\\
MCL-LOG & 46.13\scriptsize{$\pm$0.57} & & 8.57\scriptsize{$\pm$0.20} & & 15.02\scriptsize{$\pm$2.25} & & 6.55\scriptsize{$\pm$0.95} & & 5.75\\
\midrule
FWD & \bf{52.48\scriptsize{$\pm$0.63}} & & \bf{24.56\scriptsize{$\pm$0.95}} & & 29.33\scriptsize{$\pm$0.85} & & \bf{10.11\scriptsize{$\pm$1.29}} & & \bf{1.25}\\
URE-TNN & 35.60\scriptsize{$\pm$0.87} & & 9.91\scriptsize{$\pm$2.98} & & 17.98\scriptsize{$\pm$3.25} & & 8.31\scriptsize{$\pm$0.59} & & 5.25\\
URE-TGA & 45.08\scriptsize{$\pm$0.70} & & 5.83\scriptsize{$\pm$1.36} & & 17.95\scriptsize{$\pm$5.70} & & 5.78\scriptsize{$\pm$0.14} & & 5.75\\
CPE-I & 45.54\scriptsize{$\pm$2.83} & & 20.41\scriptsize{$\pm$1.44} & & 24.10\scriptsize{$\pm$2.26} & & 8.48\scriptsize{$\pm$1.37} & & 4.00\\
CPE-F & 51.74\scriptsize{$\pm$0.98} & & 24.44\scriptsize{$\pm$1.07} & & \bf{29.51\scriptsize{$\pm$0.95}} & & 9.52\scriptsize{$\pm$1.71} & & 2.00\\
CPE-T & 49.79\scriptsize{$\pm$1.45} & & 20.85\scriptsize{$\pm$0.52} & & 27.97\scriptsize{$\pm$1.06} & & 9.70\scriptsize{$\pm$1.13} & & 2.75\\
\bottomrule
\end{tabular}%
}
% }
\end{table}

==> Tables/Multi-Hard.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of test accuracies where instances have 3 CLs on Real-World datasets.}
% \vskip 0.15in
\label{tab:multi-hard}
\resizebox{1\linewidth}{!}{%
% \scalebox{0.8}{
\begin{tabular}{lcccccccccccccccc}
\toprule
& \multicolumn{2}{c}{CLCIFAR10} & & \multicolumn{2}{c}{CLCIFAR20} & & \multicolumn{2}{c}{CLMIN10} & & \multicolumn{2}{c}{CLMIN20} & & \multicolumn{2}{c}{Avg.} \\
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12} \cmidrule{14-15}
& ResNet18 & ResNet34 & & ResNet18 & ResNet34 & & ResNet18 & ResNet34 & & ResNet18 & ResNet34 & & ResNet18 & ResNet34 \\
\midrule
SCL-NL	&	43.19	&	43.50	&		&	8.14	&	10.08	&		&	14.27	&	11.65	&		&	7.59	&	\bf{7.58}	&		&	18.30	&	18.20\\
SCL-EXP	&	45.76	&	44.20	&		&	9.07	&	10.00	&		&	18.93	&	13.63	&		&	7.52	&	6.56	&		&	20.32	&	18.60\\
URE-NN	&	43.25	&	45.88	&		&	\bf{16.98}	&	\bf{14.03}	&		&	22.60	&	\bf{27.28}	&		&	8.08	&	7.36	&		&	22.73	&	\bf{23.64}\\
URE-GA	&	\bf{49.19}	&	42.20	&		&	13.60	&	9.44	&		&	\bf{23.29}	&	20.68	&		&	\bf{8.70}	&	6.30	&		&	\bf{23.70}	&	19.65\\
DM	&	40.61	&	43.30	&		&	9.18	&	9.79	&		&	16.33	&	19.76	&		&	6.76	&	7.30	&		&	18.22	&	20.04\\
MCL-MAE	&	32.75	&	18.12	&		&	8.12	&	5.78	&		&	10.99	&	10.40	&		&	5.89	&	6.72	&		&	14.44	&	10.26\\
MCL-EXP	&	43.66	&	\bf{46.02}	&		&	8.68	&	10.59	&		&	18.29	&	15.04	&		&	7.09	&	6.99	&		&	19.43	&	19.66\\
MCL-LOG	&	40.73	&	43.42	&		&	7.56	&	10.09	&		&	17.05	&	18.22	&		&	7.54	&	5.90	&		&	18.22	&	19.41\\
\midrule
FWD	&	\bf{50.88}	&	\bf{51.41}	&		&	\bf{24.78}	&	\bf{22.88}	&		&	\bf{36.88}	&	30.88	&		&	11.89	&	11.52	&		&	\bf{31.11}	&	29.17\\
URE-TNN	&	37.79	&	36.01	&		&	11.65	&	9.34	&		&	21.25	&	19.66	&		&	6.31	&	5.50	&		&	19.25	&	17.63\\
URE-TGA	&	46.73	&	44.94	&		&	6.13	&	5.39	&		&	25.56	&	27.09	&		&	4.57	&	5.30	&		&	20.75	&	20.68\\
CPE-I	&	40.55	&	43.40	&		&	15.21	&	17.24	&		&	19.93	&	24.60	&		&	8.51	&	7.91	&		&	21.05	&	23.29\\
CPE-F	&	49.86	&	50.53	&		&	23.11	&	22.56	&		&	36.11	&	31.31	&		&	11.87	&	11.32	&		&	30.24	&	28.93\\
CPE-T	&	49.71	&	50.41	&		&	23.86	&	22.77	&		&	32.67	&	\bf{32.78}	&		&	\bf{12.13}	&	\bf{11.58}	&		&	29.59	&	\bf{29.38}\\
\bottomrule
\end{tabular}%
}
% }
\end{table}

==> Tables/Multi-Simple.tex <==
\begin{table}[t]
\centering
\caption{Comparison of test accuracies where instances have 3 CLs on Synthetic datasets.}
% \vskip 0.15in
\label{tab:multi-simple}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{lccccccccccccccccccccccccccc}
\toprule
& {MNIST} & & {KMNIST} & & {FMNIST} & & {Yeast} & & {Texture} & & {Dermatology} & & {Control} & & {CIFAR10} & & {CIFAR20} & & {MIN10} & & {MIN20} &  & {Avg.} \\
\midrule
SCL-NL	&	\bf{95.67}	&		&	71.46	&		&	\bf{85.83}	&		&	47.65	&		&	95.22	&		&	97.30	&		&	60.00	&		&	76.52	&		&	33.57	&		&	53.90	&		&	23.62	&		&	67.34\\
SCL-EXP	&	95.22	&		&	70.21	&		&	85.31	&		&	44.97	&		&	95.22	&		&	97.30	&		&	58.33	&		&	76.85	&		&	33.96	&		&	\bf{54.81}	&		&	23.61	&		&	66.89\\
URE-NN	&	94.22	&		&	\bf{76.68}	&		&	85.33	&		&	33.56	&		&	77.16	&		&	\bf{100.00}	&		&	55.00	&		&	59.36	&		&	23.15	&		&	33.92	&		&	15.65	&		&	59.46\\
URE-GA	&	94.45	&		&	76.39	&		&	85.12	&		&	38.26	&		&	71.79	&		&	37.84	&		&	58.33	&		&	75.95	&		&	23.07	&		&	40.75	&		&	20.44	&		&	56.58\\
DM	&	93.51	&		&	70.11	&		&	85.31	&		&	\bf{49.66}	&		&	93.69	&		&	97.30	&		&	60.00	&		&	68.33	&		&	29.01	&		&	45.01	&		&	19.40	&		&	64.67\\
MCL-MAE	&	94.73	&		&	67.63	&		&	85.02	&		&	41.61	&		&	84.32	&		&	83.78	&		&	51.67	&		&	64.11	&		&	6.43	&		&	40.26	&		&	\bf{79.51}	&		&	63.55\\
MCL-EXP	&	95.03	&		&	70.10	&		&	85.57	&		&	46.31	&		&	95.22	&		&	97.30	&		&	55.00	&		&	77.44	&		&	32.90	&		&	53.06	&		&	21.37	&		&	66.30\\
MCL-LOG	&	95.56	&		&	71.82	&		&	85.80	&		&	48.99	&		&	\bf{95.48}	&		&	\bf{100.00}	&		&	\bf{70.00}	&		&	\bf{78.00}	&		&	\bf{34.34}	&		&	53.15	&		&	20.73	&		&	\bf{68.53}\\
\midrule
FWD	&	95.47	&		&	71.73	&		&	\bf{86.09}	&		&	\bf{53.02}	&		&	95.09	&		&	97.30	&		&	\bf{73.33}	&		&	\bf{77.41}	&		&	32.73	&		&	\bf{51.50}	&		&	21.17	&		&	\bf{68.62}\\
URE-TNN	&	94.09	&		&	\bf{77.26}	&		&	85.71	&		&	36.24	&		&	80.35	&		&	\bf{100.00}	&		&	56.67	&		&	60.87	&		&	23.15	&		&	30.49	&		&	15.34	&		&	60.02\\
URE-TGA	&	94.53	&		&	76.28	&		&	85.19	&		&	34.90	&		&	72.67	&		&	40.54	&		&	65.00	&		&	75.83	&		&	24.54	&		&	42.76	&		&	16.03	&		&	57.12\\
CPE-I	&	93.48	&		&	75.04	&		&	84.77	&		&	48.99	&		&	89.69	&		&	89.19	&		&	71.67	&		&	63.99	&		&	19.58	&		&	37.70	&		&	11.64	&		&	62.34\\
CPE-F	&	95.49	&		&	71.75	&		&	86.07	&		&	44.30	&		&	\bf{96.09}	&		&	97.30	&		&	\bf{73.33}	&		&	77.40	&		&	\bf{32.76}	&		&	51.28	&		&	21.46	&		&	67.93\\
CPE-T	&	\bf{95.63}	&		&	71.57	&		&	85.95	&		&	45.64	&		&	95.31	&		&	97.30	&		&	71.67	&		&	76.00	&		&	31.84	&		&	48.94	&		&	\bf{22.39}	&		&	67.48\\
\bottomrule
\end{tabular}%
}
\end{table}

==> Tables/Multi.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of test accuracies where instances have random number of complementary labels on Synthetic datasets.}
% \vskip 0.15in
\label{tab:multi}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{lccccccccccccccccccccccccccc}
\toprule
& {MNIST} & & {KMNIST} & & {FMNIST} & & {Yeast} & & {Texture} & & {Dermatology} & & {Control}  & & {CIFAR10} & & {CIFAR20}  & & {MIN10} & & {MIN20}  &  & {Avg.} \\
\midrule
SCL-NL	&	96.68	&		&	75.86	&		&	86.90	&		&	\bf{50.34}	&		&	94.96	&		&	97.30	&		&	55.00	&		&	\bf{81.88}	&		&	\bf{53.25}	&		&	58.16	&		&	\bf{49.60}	&		&	72.72\\
SCL-EXP	&	96.18	&		&	74.27	&		&	86.46	&		&	45.64	&		&	94.70	&		&	97.30	&		&	55.00	&		&	81.18	&		&	53.09	&		&	57.22	&		&	49.27	&		&	71.85\\
URE-NN	&	94.23	&		&	76.84	&		&	85.36	&		&	28.19	&		&	84.96	&		&	89.19	&		&	56.67	&		&	55.96	&		&	32.27	&		&	38.90	&		&	23.24	&		&	60.53\\
URE-GA	&	94.97	&		&	78.02	&		&	85.72	&		&	34.23	&		&	77.29	&		&	86.49	&		&	55.00	&		&	79.53	&		&	42.99	&		&	39.82	&		&	26.53	&		&	63.69\\
DM	&	95.89	&		&	74.87	&		&	86.76	&		&	46.98	&		&	95.22	&		&	\bf{100.00}	&		&	60.00	&		&	77.19	&		&	48.66	&		&	51.83	&		&	42.31	&		&	70.88\\
MCL-MAE	&	95.99	&		&	71.53	&		&	85.45	&		&	28.19	&		&	89.17	&		&	83.78	&		&	35.00	&		&	75.57	&		&	23.55	&		&	43.63	&		&	19.01	&		&	59.17\\
MCL-EXP	&	96.19	&		&	72.97	&		&	86.37	&		&	40.27	&		&	95.09	&		&	97.30	&		&	53.33	&		&	80.20	&		&	52.17	&		&	\bf{60.39}	&		&	46.33	&		&	70.96\\
MCL-LOG	&	\bf{96.87}	&		&	\bf{83.99}	&		&	\bf{87.05}	&		&	48.32	&		&	\bf{95.74}	&		&	97.30	&		&	\bf{63.33}	&		&	81.04	&		&	52.62	&		&	60.36	&		&	47.70	&		&	\bf{74.03}\\
\midrule
FWD	&	96.63	&		&	76.11	&		&	\bf{87.09}	&		&	\bf{56.38}	&		&	\bf{95.35}	&		&	\bf{97.30}	&		&	\bf{70.00}	&		&	81.75	&		&	52.58	&		&	\bf{59.34}	&		&	\bf{49.67}	&		&	\bf{74.75}\\
URE-TNN	&	94.25	&		&	76.87	&		&	85.37	&		&	38.26	&		&	83.73	&		&	94.59	&		&	68.33	&		&	54.56	&		&	31.38	&		&	52.96	&		&	38.34	&		&	65.33\\
URE-TGA	&	95.06	&		&	77.48	&		&	85.75	&		&	36.24	&		&	79.95	&		&	94.59	&		&	63.33	&		&	78.94	&		&	41.98	&		&	50.52	&		&	36.59	&		&	67.31\\
CPE-I	&	95.37	&		&	\bf{78.54}	&		&	86.04	&		&	50.34	&		&	91.18	&		&	91.89	&		&	53.33	&		&	73.49	&		&	37.29	&		&	45.64	&		&	25.58	&		&	66.24\\
CPE-F	&	96.63	&		&	76.08	&		&	87.07	&		&	46.98	&		&	95.22	&		&	94.59	&		&	61.67	&		&	81.73	&		&	52.57	&		&	\bf{59.34}	&		&	\bf{49.67}	&		&	72.87\\
CPE-T	&	\bf{96.66}	&		&	75.30	&		&	87.06	&		&	42.95	&		&	95.09	&		&	94.59	&		&	60.00	&		&	\bf{81.91}	&		&	\bf{52.82}	&		&	58.18	&		&	46.74	&		&	71.94\\
\bottomrule
\end{tabular}%
}
\end{table}

==> Tables/Noisy.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of testing accuracies with different levels of noise in transition matrices. $\lambda$ stands for the weights between uniform noise transition matrix $\frac{1}{K}1_K$ and Strong deviation transition matrix. Datasets with higher $\lambda$ are noisier.}
% \vskip 0.15in
\label{tab:noisy}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lcccccccccccccccccccccccc}
\toprule
& \multicolumn{3}{c}{MNIST} & & \multicolumn{3}{c}{KMNIST} & & \multicolumn{3}{c}{FMNIST} & & \multicolumn{3}{c}{CIFAR10} & & \multicolumn{3}{c}{MIN10} & & \multicolumn{3}{c}{Avg.} \\
\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} \cmidrule{14-16} \cmidrule{18-20} \cmidrule{22-24}
& \lambda = 0.1 & \lambda = 0.2 & \lambda = 0.5 & & \lambda = 0.1 & \lambda = 0.2 & \lambda = 0.5 & & \lambda = 0.1 & \lambda = 0.2 & \lambda = 0.5 & & \lambda = 0.1 & \lambda = 0.2 & \lambda = 0.5 & & \lambda = 0.1 & \lambda = 0.2 & \lambda = 0.5 & & \lambda = 0.1 & \lambda = 0.2 & \lambda = 0.5 \\
\midrule
SCL-NL	&	19.92	&	22.51	&	16.22	&		&	18.13	&	18.17	&	20.17	&		&	23.19	&	17.05	&	23.32	&		&	22.78	&	21.38	&	20.33	&		&	23.87	&	18.30	&	17.89	&		&	21.58	&	19.48	&	19.59\\
SCL-EXP	&	23.57	&	20.50	&	15.25	&		&	18.71	&	17.24	&	\bf{20.69}	&		&	24.39	&	18.18	&	15.70	&		&	24.44	&	23.70	&	22.65	&		&	25.95	&	22.56	&	15.17	&		&	23.41	&	20.44	&	17.89\\
URE-NN	&	\bf{29.73}	&	\bf{34.42}	&	\bf{25.90}	&		&	18.99	&	21.74	&	17.84	&		&	\bf{39.89}	&	\bf{35.56}	&	\bf{29.46}	&		&	\bf{27.56}	&	\bf{31.79}	&	23.28	&		&	18.16	&	18.75	&	16.67	&		&	\bf{26.87}	&	\bf{28.45}	&	\bf{22.63}\\
URE-GA	&	29.65	&	23.59	&	13.18	&		&	16.39	&	16.56	&	18.79	&		&	29.23	&	22.54	&	19.72	&		&	24.86	&	26.46	&	\bf{25.36}	&		&	\bf{28.30}	&	\bf{24.78}	&	\bf{19.52}	&		&	25.69	&	22.79	&	19.31\\
DM	&	27.00	&	24.99	&	20.47	&		&	\bf{22.63}	&	\bf{22.21}	&	18.93	&		&	26.95	&	28.54	&	27.38	&		&	24.38	&	23.71	&	21.57	&		&	20.58	&	18.17	&	12.68	&		&	24.31	&	23.52	&	20.21\\
\midrule
FWD	&	95.07	&	94.37	&	87.03	&		&	\bf{77.12}	&	\bf{74.14}	&	60.81	&		&	\bf{85.23}	&	83.74	&	75.90	&		&	68.41	&	65.38	&	47.42	&		&	47.71	&	43.12	&	27.81	&		&	\bf{74.71}	&	72.15	&	59.79\\
URE-TNN	&	85.45	&	84.30	&	78.98	&		&	62.79	&	60.33	&	50.61	&		&	80.81	&	79.59	&	74.17	&		&	47.78	&	45.62	&	32.17	&		&	24.67	&	24.34	&	14.86	&		&	60.30	&	58.84	&	50.16\\
URE-TGA	&	89.04	&	87.76	&	79.76	&		&	67.60	&	66.13	&	51.41	&		&	82.43	&	80.82	&	76.23	&		&	61.98	&	53.10	&	38.38	&		&	37.22	&	34.62	&	29.08	&		&	67.65	&	64.49	&	54.97\\
CPE-I	&	92.66	&	92.21	&	89.35	&		&	74.12	&	71.26	&	64.38	&		&	83.67	&	83.15	&	\bf{81.34}	&		&	63.58	&	61.05	&	48.59	&		&	42.93	&	36.21	&	30.55	&		&	71.39	&	68.78	&	62.84\\
CPE-F	&	95.04	&	\bf{94.42}	&	\bf{90.47}	&		&	76.65	&	74.08	&	65.06	&		&	84.61	&	\bf{84.11}	&	81.09	&		&	\bf{68.51}	&	\bf{65.50}	&	\bf{52.03}	&		&	46.13	&	44.36	&	23.05	&		&	74.19	&	\bf{72.49}	&	62.34\\
CPE-T	&	\bf{95.14}	&	94.36	&	90.41	&		&	75.84	&	73.68	&	\bf{65.41}	&		&	84.60	&	84.10	&	80.93	&		&	67.41	&	64.37	&	51.48	&		&	\bf{50.47}	&	\bf{45.36}	&	\bf{32.65}	&		&	74.69	&	72.37	&	\bf{64.18}\\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/Uniform-Hard-New.tex <==
\begin{table}[ht]
% \begin{minipage}[!t]{\columnwidth}
\centering
\caption{Baseline testing accuracies of strategies on Real-World datasets.}
% \vskip 0.15in
\label{tab:hard}
% \resizebox{1\linewidth}{!}{%
\scalebox{0.85}{
\begin{tabular}{lcccccccccccccccc}
\toprule
% & \multicolumn{2}{c}{CLCIFAR10} & \multicolumn{2}{c}{CLCIFAR20} & \multicolumn{2}{c}{CLMIN10} & \multicolumn{2}{c}{CLMIN20} & \multicolumn{2}{c}{Avg.} \\
& {CLCIFAR10} & {CLCIFAR20} & {CLMIN10} & {CLMIN20} & {Avg Rank} \\
% \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12} \cmidrule{14-15}
% & ResNet18 & ResNet34 & ResNet18 & ResNet34 & ResNet18 & ResNet34 & ResNet18 & ResNet34 & ResNet18 & ResNet34 \\
\midrule
SCL-NL & 36.21\scriptsize{$\pm$2.06} & 7.92\scriptsize{$\pm$0.23} & 16.59\scriptsize{$\pm$3.46} & \bf{6.82\scriptsize{$\pm$0.53}} & \bf{2.25}\\
SCL-EXP & 35.95\scriptsize{$\pm$1.97} & 7.79\scriptsize{$\pm$0.06} & 12.60\scriptsize{$\pm$0.58} & 5.81\scriptsize{$\pm$0.86} & 4.75\\
URE-NN & 34.66\scriptsize{$\pm$1.64} & \bf{11.77\scriptsize{$\pm$0.72}} & \bf{19.51\scriptsize{$\pm$3.21}} & 4.93\scriptsize{$\pm$0.42} & 4.00\\
URE-GA & 37.32\scriptsize{$\pm$0.61} & 7.09\scriptsize{$\pm$0.77} & 14.34\scriptsize{$\pm$2.48} & 5.99\scriptsize{$\pm$0.92} & 3.50\\
DM & 36.78\scriptsize{$\pm$0.81} & 7.66\scriptsize{$\pm$0.10} & 14.03\scriptsize{$\pm$1.69} & 5.48\scriptsize{$\pm$0.74} & 4.50\\
MCL-MAE & 20.01\scriptsize{$\pm$1.41} & 6.55\scriptsize{$\pm$0.76} & 11.94\scriptsize{$\pm$1.00} & 5.78\scriptsize{$\pm$0.54} & 7.25\\
MCL-EXP & 34.54\scriptsize{$\pm$1.09} & 7.82\scriptsize{$\pm$0.23} & 13.75\scriptsize{$\pm$2.39} & 5.43\scriptsize{$\pm$1.03} & 5.75\\
MCL-LOG & \bf{37.35\scriptsize{$\pm$1.17}} & 7.49\scriptsize{$\pm$0.39} & 13.93\scriptsize{$\pm$2.75} & 5.79\scriptsize{$\pm$0.47} & 4.00\\
\midrule
FWD & \bf{39.25\scriptsize{$\pm$1.55}} & \bf{19.82\scriptsize{$\pm$0.38}} & 29.63\scriptsize{$\pm$2.92} & \bf{10.58\scriptsize{$\pm$1.14}} & \bf{1.25}\\
URE-TNN & 31.21\scriptsize{$\pm$1.11} & 9.47\scriptsize{$\pm$2.67} & 17.87\scriptsize{$\pm$4.33} & 6.30\scriptsize{$\pm$0.96} & 5.50\\
URE-TGA & 33.68\scriptsize{$\pm$1.06} & 5.17\scriptsize{$\pm$0.25} & 21.35\scriptsize{$\pm$4.38} & 5.88\scriptsize{$\pm$1.21} & 5.25\\
CPE-I & 33.94\scriptsize{$\pm$1.40} & 16.79\scriptsize{$\pm$0.48} & 20.18\scriptsize{$\pm$4.25} & 8.61\scriptsize{$\pm$0.43} & 4.25\\
CPE-F & 38.94\scriptsize{$\pm$1.39} & 19.48\scriptsize{$\pm$0.35} & \bf{29.82\scriptsize{$\pm$3.13}} & 10.16\scriptsize{$\pm$0.84} & 1.75\\
CPE-T & 38.80\scriptsize{$\pm$1.16} & 19.33\scriptsize{$\pm$0.75} & 28.85\scriptsize{$\pm$0.55} & 9.36\scriptsize{$\pm$1.32} & 3.00\\
\bottomrule
\end{tabular}
}
% \end{minipage}
\end{table}
% \begin{table}[ht]
% \centering
% \caption{Baseline testing accuracies of strategies on Real-World and Synthetic datasets.}
% \label{tab:combined}
% \scalebox{0.68}{
% \begin{tabular}{lcccccccccccccccccccccccccc}
% \toprule
% & \multicolumn{5}{c}{Real-World Datasets} & \multicolumn{5}{c}{Synthetic Datasets} \\
% \cmidrule(lr){2-6} \cmidrule(lr){7-11}
% Method & {CLCIFAR10} & {CLCIFAR20} & {CLMIN10} & {CLMIN20} & {Avg Rank} 
% & {Yeast} & {Texture} & {Dermatology} & {Control} & {Avg Rank} \\
% \midrule
% SCL-NL & 36.21\scriptsize{$\pm$2.06} & 7.92\scriptsize{$\pm$0.23} & 16.59\scriptsize{$\pm$3.46} & \bf{6.82\scriptsize{$\pm$0.53}} & \bf{2.25} 
% & 49.33\scriptsize{$\pm$5.46} & 97.22\scriptsize{$\pm$0.83} & 72.97\scriptsize{$\pm$6.04} & 77.50\scriptsize{$\pm$10.57} & 3.25 \\
% SCL-EXP & 35.95\scriptsize{$\pm$1.97} & 7.79\scriptsize{$\pm$0.06} & 12.60\scriptsize{$\pm$0.58} & 5.81\scriptsize{$\pm$0.86} & 4.75
% & 47.15\scriptsize{$\pm$6.44} & \bf{97.40\scriptsize{$\pm$0.79}} & 70.27\scriptsize{$\pm$6.62} & 77.08\scriptsize{$\pm$11.39} & 4.38 \\
% URE-NN & 34.66\scriptsize{$\pm$1.64} & \bf{11.77\scriptsize{$\pm$0.72}} & \bf{19.51\scriptsize{$\pm$3.21}} & 4.93\scriptsize{$\pm$0.42} & 4.00
% & 48.66\scriptsize{$\pm$2.15} & 86.95\scriptsize{$\pm$3.77} & \bf{85.14\scriptsize{$\pm$2.34}} & 51.25\scriptsize{$\pm$6.17} & 4.25 \\
% URE-GA & 37.32\scriptsize{$\pm$0.61} & 7.09\scriptsize{$\pm$0.77} & 14.34\scriptsize{$\pm$2.48} & 5.99\scriptsize{$\pm$0.92} & 3.50
% & 47.82\scriptsize{$\pm$3.33} & 79.59\scriptsize{$\pm$5.87} & 79.05\scriptsize{$\pm$6.16} & 45.42\scriptsize{$\pm$5.45} & 5.25 \\
% DM & 36.78\scriptsize{$\pm$0.81} & 7.66\scriptsize{$\pm$0.10} & 14.03\scriptsize{$\pm$1.69} & 5.48\scriptsize{$\pm$0.74} & 4.50
% & 34.73\scriptsize{$\pm$7.45} & 95.34\scriptsize{$\pm$1.32} & 70.27\scriptsize{$\pm$6.89} & \bf{78.75\scriptsize{$\pm$8.53}} & 4.88 \\
% MCL-MAE & 20.01\scriptsize{$\pm$1.41} & 6.55\scriptsize{$\pm$0.76} & 11.94\scriptsize{$\pm$1.00} & 5.78\scriptsize{$\pm$0.54} & 7.25
% & 33.72\scriptsize{$\pm$5.66} & 60.51\scriptsize{$\pm$9.40} & 66.22\scriptsize{$\pm$11.55} & 43.33\scriptsize{$\pm$7.73} & 8.00 \\
% MCL-EXP & 34.54\scriptsize{$\pm$1.09} & 7.82\scriptsize{$\pm$0.23} & 13.75\scriptsize{$\pm$2.39} & 5.43\scriptsize{$\pm$1.03} & 5.75
% & 51.01\scriptsize{$\pm$6.49} & 97.28\scriptsize{$\pm$1.00} & 73.65\scriptsize{$\pm$5.85} & 77.50\scriptsize{$\pm$10.96} & \bf{2.62} \\
% MCL-LOG & \bf{37.35\scriptsize{$\pm$1.17}} & 7.49\scriptsize{$\pm$0.39} & 13.93\scriptsize{$\pm$2.75} & 5.79\scriptsize{$\pm$0.47} & 4.00
% & \bf{55.37\scriptsize{$\pm$6.30}} & 96.93\scriptsize{$\pm$1.05} & 73.65\scriptsize{$\pm$7.73} & 76.67\scriptsize{$\pm$7.55} & 3.38 \\
% \midrule
% FWD & \bf{39.25\scriptsize{$\pm$1.55}} & \bf{19.82\scriptsize{$\pm$0.38}} & 29.63\scriptsize{$\pm$2.92} & \bf{10.58\scriptsize{$\pm$1.14}} & \bf{1.25}
% & \bf{58.72\scriptsize{$\pm$3.17}} & \bf{97.12\scriptsize{$\pm$0.75}} & 79.05\scriptsize{$\pm$9.63} & \bf{90.83\scriptsize{$\pm$6.72}} & \bf{1.75} \\
% URE-TNN & 31.21\scriptsize{$\pm$1.11} & 9.47\scriptsize{$\pm$2.67} & 17.87\scriptsize{$\pm$4.33} & 6.30\scriptsize{$\pm$0.96} & 5.50
% & 37.75\scriptsize{$\pm$14.53} & 88.01\scriptsize{$\pm$3.08} & 81.08\scriptsize{$\pm$3.82} & 62.92\scriptsize{$\pm$5.45} & 4.00 \\
% URE-TGA & 33.68\scriptsize{$\pm$1.06} & 5.17\scriptsize{$\pm$0.25} & 21.35\scriptsize{$\pm$4.38} & 5.88\scriptsize{$\pm$1.21} & 5.25
% & 35.57\scriptsize{$\pm$15.60} & 81.42\scriptsize{$\pm$2.74} & 78.38\scriptsize{$\pm$5.06} & 58.75\scriptsize{$\pm$6.28} & 6.00 \\
% CPE-I & 33.94\scriptsize{$\pm$1.40} & 16.79\scriptsize{$\pm$0.48} & 20.18\scriptsize{$\pm$4.25} & 8.61\scriptsize{$\pm$0.43} & 4.25
% & 52.68\scriptsize{$\pm$1.93} & 91.39\scriptsize{$\pm$0.86} & \bf{81.76\scriptsize{$\pm$5.85}} & 59.17\scriptsize{$\pm$13.15} & 3.50 \\
% CPE-F & 38.94\scriptsize{$\pm$1.39} & 19.48\scriptsize{$\pm$0.71} & \bf{29.71\scriptsize{$\pm$3.89}} & 10.20\scriptsize{$\pm$0.64} & 1.75
% & 54.74\scriptsize{$\pm$5.16} & 96.69\scriptsize{$\pm$0.77} & 78.65\scriptsize{$\pm$7.09} & 88.75\scriptsize{$\pm$5.34} & \bf{2.00} \\
% \bottomrule
% \end{tabular}}
% \end{table}


==> Tables/Uniform-Hard.tex <==
\begin{table}[ht]
\centering
\caption{Baseline testing accuracies of strategies on Real-World datasets.}
% \vskip 0.15in
\label{tab:hard}
\resizebox{1\linewidth}{!}{%
% \scalebox{0.6}{
\begin{tabular}{lcccccccccccccccc}
\toprule
& \multicolumn{2}{c}{CLCIFAR10} & & \multicolumn{2}{c}{CLCIFAR20} & & \multicolumn{2}{c}{CLMIN10} & & \multicolumn{2}{c}{CLMIN20} & & \multicolumn{2}{c}{Avg.} \\
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12} \cmidrule{14-15}
& ResNet18 & ResNet34 & & ResNet18 & ResNet34 & & ResNet18 & ResNet34 & & ResNet18 & ResNet34 & & ResNet18 & ResNet34 \\
\midrule
SCL-NL	&	37.53	&	35.99	&		&	7.97	&	8.53	&		&	\bf{20.79}	&	17.07	&		&	6.35	&	6.49	&		&	\bf{18.16}	&	17.02\\
SCL-EXP	&	36.89	&	36.11	&		&	8.33	&	7.49	&		&	17.95	&	13.35	&		&	\bf{6.91}	&	6.51	&		&	17.52	&	15.87\\
URE-NN	&	35.60	&	36.99	&		&	\bf{11.70}	&	\bf{12.12}	&		&	19.15	&	\bf{23.30}	&		&	5.59	&	\bf{7.26}	&		&	18.01	&	\bf{19.92}\\
URE-GA	&	\bf{38.92}	&	\bf{39.66}	&		&	6.80	&	8.76	&		&	16.95	&	14.41	&		&	6.00	&	5.96	&		&	17.17	&	17.20\\
DM	&	36.40	&	35.70	&		&	8.26	&	8.59	&		&	16.47	&	14.98	&		&	6.72	&	5.64	&		&	16.96	&	16.23\\
MCL-MAE	&	27.47	&	16.96	&		&	8.48	&	8.00	&		&	12.17	&	10.68	&		&	5.28	&	5.74	&		&	13.35	&	10.35\\
MCL-EXP	&	36.70	&	38.13	&		&	7.79	&	7.43	&		&	16.90	&	14.89	&		&	5.49	&	6.39	&		&	16.72	&	16.71\\
MCL-LOG	&	35.87	&	34.21	&		&	8.07	&	8.33	&		&	16.79	&	20.08	&		&	5.21	&	5.48	&		&	16.48	&	17.02\\
\midrule
FWD	&	39.63	&	\bf{39.08}	&		&	19.60	&	18.64	&		&	33.59	&	29.23	&		&	9.49	&	8.13	&		&	25.58	&	23.77\\
URE-TNN	&	31.03	&	28.77	&		&	10.56	&	6.24	&		&	18.71	&	16.79	&		&	7.13	&	7.38	&		&	16.86	&	14.79\\
URE-TGA	&	36.08	&	36.70	&		&	5.02	&	5.72	&		&	21.80	&	19.36	&		&	4.88	&	4.88	&		&	16.94	&	16.66\\
CPE-I	&	33.81	&	32.71	&		&	13.96	&	13.46	&		&	26.16	&	21.85	&		&	6.00	&	6.54	&		&	19.98	&	18.64\\
CPE-F	&	39.52	&	38.94	&		&	\bf{20.30}	&	\bf{18.69}	&		&	30.50	&	30.05	&		&	10.75	&	\bf{10.45}	&		&	25.27	&	\bf{24.53}\\
CPE-T	&	\bf{39.76}	&	38.00	&		&	19.82	&	18.56	&		&	\bf{34.64}	&	\bf{30.11}	&		&	\bf{11.10}	&	8.03	&		&	\bf{26.33}	&	23.68\\
\bottomrule
\end{tabular}
}
% }
\end{table}

==> Tables/Uniform-Simple.tex <==
\begin{table}[ht]
\centering
\caption{Baseline testing accuracies of strategies with uniform distribution on Synthetic datasets.}
% \vskip 0.15in
\label{tab:simple}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{lcccccccccccccccccccccccccc}
\toprule
& {MNIST} & & {KMNIST} & & {FMNIST} & & {Yeast} & & {Texture} & & {Dermatology} & & {Control} & & {CIFAR10} & & {CIFAR20} & & {MIN10} & & {MIN20} & & Avg.\\
\midrule
SCL-NL	&	92.17	&		&	63.90	&		&	83.30	&		&	47.65	&		&	86.76	&		&	67.57	&		&	48.33	&		&	62.64	&		&	20.30	&		&	\bf{39.09}	&		&	10.89	&		&	56.60\\
SCL-EXP	&	91.90	&		&	63.28	&		&	83.22	&		&	46.98	&		&	84.94	&		&	70.27	&		&	45.00	&		&	\bf{64.76}	&		&	20.56	&		&	36.89	&		&	\bf{13.57}	&		&	56.49\\
URE-NN	&	91.66	&		&	68.26	&		&	82.00	&		&	31.54	&		&	56.61	&		&	70.27	&		&	\bf{50.00}	&		&	41.50	&		&	16.01	&		&	24.06	&		&	11.42	&		&	49.39\\
URE-GA	&	\bf{92.96}	&		&	\bf{70.50}	&		&	83.13	&		&	27.52	&		&	56.87	&		&	51.35	&		&	48.33	&		&	60.86	&		&	16.79	&		&	31.40	&		&	7.96	&		&	49.79\\
DM	&	91.34	&		&	66.40	&		&	83.46	&		&	48.32	&		&	87.64	&		&	\bf{78.38}	&		&	48.83	&		&	56.47	&		&	18.46	&		&	31.33	&		&	12.37	&		&	\bf{56.64}\\
MCL-MAE	&	91.83	&		&	58.60	&		&	82.72	&		&	28.19	&		&	42.16	&		&	64.86	&		&	35.00	&		&	33.59	&		&	5.86	&		&	17.77	&		&	8.25	&		&	42.62\\
MCL-EXP	&	91.91	&		&	63.21	&		&	\bf{83.55}	&		&	\bf{48.99}	&		&	85.59	&		&	64.86	&		&	45.00	&		&	63.37	&		&	\bf{22.36}	&		&	35.87	&		&	10.82	&		&	55.96\\
MCL-LOG	&	92.23	&		&	63.95	&		&	83.37	&		&	48.32	&		&	\bf{88.55}	&		&	64.86	&		&	46.67	&		&	62.66	&		&	20.91	&		&	37.51	&		&	12.46	&		&	56.50\\
FWD	&	89.25	&		&	64.10	&		&	\bf{83.31}	&		&	37.57	&		&	\bf{90.56}	&		&	83.78	&		&	40.00	&		&	\bf{62.91}	&		&	19.14	&		&	\bf{38.03}	&		&	\bf{15.43}	&		&	56.73\\
URE-TNN	&	91.84	&		&	68.55	&		&	82.25	&		&	24.83	&		&	62.39	&		&	72.97	&		&	48.33	&		&	39.91	&		&	15.23	&		&	30.54	&		&	9.96	&		&	49.71\\
URE-TGA	&	\bf{92.72}	&		&	\bf{71.01}	&		&	82.81	&		&	24.83	&		&	55.95	&		&	72.97	&		&	46.67	&		&	59.55	&		&	14.80	&		&	35.14	&		&	5.26	&		&	51.06\\
CPE-I	&	90.44	&		&	66.22	&		&	80.90	&		&	\bf{41.61}	&		&	72.64	&		&	78.38	&		&	\bf{70.00}	&		&	43.38	&		&	12.61	&		&	26.14	&		&	7.39	&		&	53.61\\
CPE-F	&	92.16	&		&	64.10	&		&	83.23	&		&	37.58	&		&	88.25	&		&	\bf{86.49}	&		&	61.67	&		&	62.89	&		&	19.17	&		&	38.01	&		&	15.41	&		&	\bf{59.00}\\
CPE-T	&	91.90	&		&	63.90	&		&	83.17	&		&	34.23	&		&	79.50	&		&	\bf{86.49}	&		&	\bf{70.00}	&		&	60.62	&		&	\bf{19.79}	&		&	36.08	&		&	13.62	&		&	58.12\\
\bottomrule
\end{tabular}%
}
\end{table}

==> Tables/autoaugment.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of performance using \textbf{AutoAugment} on CLCIFAR and uniform-CIFAR datasets in relation to tab:exp-1. The accuracy changes are shown in subscript, with enhanced accuracy values being highlighted in bold.}
\label{tab:autoaug}
%vskip 0.05in
\resizebox{\columnwidth}{!}{%
\begin{small}
\begin{tabular}{lcccccccc}
\toprule
         & \multicolumn{2}{c}{uniform-CIFAR10} & \multicolumn{2}{c}{CLCIFAR10} & \multicolumn{2}{c}{uniform-CIFAR20} & \multicolumn{2}{c}{CLCIFAR20} \\ \midrule
methods  & valid\_acc     & valid\_acc (ES)    & valid\_acc  & valid\_acc (ES) & valid\_acc     & valid\_acc (ES)    & valid\_acc  & valid\_acc (ES) \\ \midrule
FWD-U & \textbf{75.72\scriptsize{$+$6.55}} & \textbf{77.02\scriptsize{$+$7.23}} & \textbf{42.46\scriptsize{$+$8.37}} & \textbf{43.52\scriptsize{$+$6.69}} & \textbf{26.8\scriptsize{$+$6.56}} & \textbf{26.93\scriptsize{$+$6.31}} & 7.38\scriptsize{$-$0.09} & \textbf{8.76\scriptsize{$+$0.49}}\\
FWD-R & \textbf{75.53\scriptsize{$+$5.79}} & \textbf{76.06\scriptsize{$+$6.47}} & \textbf{40.37\scriptsize{$+$11.49}} & \textbf{42.13\scriptsize{$+$3.23}} & \textbf{26.74\scriptsize{$+$6.74}} & \textbf{26.98\scriptsize{$+$6.27}} & \textbf{20.71\scriptsize{$+$4.57}} & \textbf{24.77\scriptsize{$+$4.46}}\\
URE-GA-U & \textbf{60.24\scriptsize{$+$5.62}} & \textbf{59.9\scriptsize{$+$4.96}} & \textbf{37.78\scriptsize{$+$3.19}} & \textbf{38.48\scriptsize{$+$2.09}} & \textbf{17.08\scriptsize{$+$1.67}} & \textbf{18.59\scriptsize{$+$2.0}} & \textbf{8.88\scriptsize{$+$1.29}} & 9.7\scriptsize{$-$0.36}\\
URE-GA-R & \textbf{58.36\scriptsize{$+$5.06}} & \textbf{59.42\scriptsize{$+$2.40}} & \textbf{31.98\scriptsize{$+$3.28}} & \textbf{33.08\scriptsize{$+$2.14}} & \textbf{18.2\scriptsize{$+$3.34}} & \textbf{19.72\scriptsize{$+$2.39}} & \textbf{10.85\scriptsize{$+$5.61}} & \textbf{9.89\scriptsize{$+$4.43}}\\
SCL-NL & \textbf{76.6\scriptsize{$+$9.45}} & \textbf{76.83\scriptsize{$+$8.19}} & \textbf{38.4\scriptsize{$+$4.6}} & \textbf{43.22\scriptsize{$+$5.41}} & \textbf{23.11\scriptsize{$+$3.07}} & \textbf{26.62\scriptsize{$+$5.94}} & 7.34\scriptsize{$-$0.24} & 8.34\scriptsize{$-$0.19}\\
SCL-EXP & \textbf{75.9\scriptsize{$+$11.04}} & \textbf{75.75\scriptsize{$+$10.35}} & \textbf{40.95\scriptsize{$+$6.36}} & \textbf{41.63\scriptsize{$+$4.67}} & \textbf{24.96\scriptsize{$+$5.56}} & \textbf{26.64\scriptsize{$+$5.61}} & 7.21\scriptsize{$-$0.34} & \textbf{8.47\scriptsize{$+$0.36}}\\
L-W & \textbf{67.2\scriptsize{$+$10.99}} & \textbf{71.07\scriptsize{$+$11.89}} & \textbf{33.89\scriptsize{$+$5.85}} & \textbf{38.16\scriptsize{$+$3.61}} & \textbf{22.28\scriptsize{$+$7.93}} & \textbf{23.19\scriptsize{$+$4.08}} & \textbf{7.58\scriptsize{$+$0.5}} & 8.64\scriptsize{$-$0.1}\\
L-UW & \textbf{72.39\scriptsize{$+$11.51}} & \textbf{73.26\scriptsize{$+$10.83}} & \textbf{34.61\scriptsize{$+$3.98}} & \textbf{40.3\scriptsize{$+$5.17}} & \textbf{23.31\scriptsize{$+$7.3}} & \textbf{24.41\scriptsize{$+$4.99}} & \textbf{7.47\scriptsize{$+$0.11}} & \textbf{8.96\scriptsize{$+$0.25}}\\
PC-sigmoid & \textbf{45.72\scriptsize{$+$17.52}} & \textbf{46.53\scriptsize{$+$7.24}} & \textbf{33.24\scriptsize{$+$8.86}} & \textbf{40.72\scriptsize{$+$4.84}} & \textbf{12.81\scriptsize{$+$3.09}} & 13.84\scriptsize{$-$2.61} & \textbf{14.15\scriptsize{$+$4.88}} & \textbf{17.06\scriptsize{$+$2.8}}\\
MAE & \textbf{61.26\scriptsize{$+$3.89}} & \textbf{63.41\scriptsize{$+$4.91}} & \textbf{21.74\scriptsize{$+$5.44}} & \textbf{23.65\scriptsize{$+$4.21}} & \textbf{20.03\scriptsize{$+$3.41}} & \textbf{21.79\scriptsize{$+$4.16}} & \textbf{5.18\scriptsize{$+$0.07}} & \textbf{6.68\scriptsize{$+$0.81}}\\
\bottomrule
\end{tabular}%
\end{small}
}
\end{table}

==> Tables/clcifar-n.tex <==
\begin{table}[t]
\centering
\caption{Benchmark results on CLCIFAR-N datasets. The classification accuracy difference is calculated by subtracting the practical CLCIFAR dataset from the performance on the synthetic CLCIFAR-N dataset.}
% \vskip 0.15in
\label{tab:clcifar-n}
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{lcc|cc}
\toprule
           & CLCIFAR10-N & diff($\downarrow$)  & CLCIFAR20-N & diff($\downarrow$)  \\
\midrule
FWD-U      & 37.1        & 2.2   & \textbf{7.58}        & 0.11  \\
FWD-R      & -           & -     & -           & -     \\
URE-GA-U   & 31.29       & -3.3  & 8.1         & 0.5   \\
URE-GA-R   & -           & -     & -           & -     \\
SCL-NL     & 37.79       & 2.06  & 7.75        & 0.16  \\
SCL-EXP    & 35.86       & 3.19  & 6.95        & -0.59 \\
L-W        & 30.1        & 2.06  & 6.16        & -0.91 \\
L-UW       & 32.69       & 2.05  & 6.89        & -0.47 \\
PC-sigmoid & 19.64       & -4.73 & 6.54        & -2.72 \\
\midrule
CCE        & 32.34 & 13.45 & 5.71 & 0.71 \\
MAE        & \textbf{41.34} & 23.09 & 6.83 & 1.83 \\
WMAE       & 37.62 & 22.26 & 6.36 & 1.08 \\
GCE        & 35.00 & 18.71 & 6.7 & 1.7 \\
SL         & 29.98 & 12.29 & 6.08 & 1.05 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> Tables/iid-result.tex <==
\begin{table}[t]
\centering
\caption{Mean accuracy difference ($\pm$ standard deviation) of different CLL algorithms. A plus indicates the performance on  is calculated as CLCIFAR-\textit{i.i.d.} accuracy minus CLCIFAR accuracy.}
% \vskip 0.05in
\label{tab:exp-feat}
\resizebox{\columnwidth}{!}{%
\begin{small}
\begin{tabular}{lccccccccc}
\toprule
    & FWD-U & FWD-R & URE-GA-U & URE-GA-R & SCL-NL & SCL-EXP & L-W & L-UW & PC-sigmoid \\
\midrule
\textit{CLCIFAR10-iid} & -1.1\scriptsize{$\pm$2.17} & -0.36\scriptsize{$\pm$1.15} & -3.03\scriptsize{$\pm$1.25} & 0.74\scriptsize{$\pm$0.35} & -0.67\scriptsize{$\pm$1.81} & -1.97\scriptsize{$\pm$1.16} & -2.5\scriptsize{$\pm$0.56} & -3.53\scriptsize{$\pm$1.36} & -2.03\scriptsize{$\pm$2.05} \\
\textit{CLCIFAR20-iid} & -0.64\scriptsize{$\pm$0.39} & -3.53\scriptsize{$\pm$1.13} & -0.37\scriptsize{$\pm$0.51} & 1.79\scriptsize{$\pm$2.34} & -0.28\scriptsize{$\pm$0.61} & -0.39\scriptsize{$\pm$0.69} & -0.5\scriptsize{$\pm$1.37} & -0.82\scriptsize{$\pm$0.04} & -2.24\scriptsize{$\pm$0.52} \\
\bottomrule
\end{tabular}%
\end{small}
}
% \vskip -0.2in
\end{table}

==> Tables/multiple-cl.tex <==
            \begin{table}[t]
\centering
\caption{Learning with Multiple CL: The figure shows the classification accuracy of each task with early stopping indicated in brackets. The highest accuracy in each column is bolded for ease of comparison.}
\label{tab:mcl}
% \vskip 0.15in
\resizebox{0.8\columnwidth}{!}{%
\begin{small}
\begin{tabular}{lccccccc}
\toprule
& \multicolumn{3}{c}{CLCIFAR10} & \multicolumn{3}{c}{CLCIFAR20} \\
\midrule
num CL  & 1 & 2 & 3 & 1 & 2 & 3 \\
\midrule
FWD-U & 34.09\scriptsize{(36.83)} & 41.95\scriptsize{(41.53)} &  42.88\scriptsize{(45.18)}        & 7.47\scriptsize{(8.27)} & 8.28\scriptsize{(8.78)} &   8.15\scriptsize{(10.27)} \\
FWD-R & 28.88\scriptsize{(\textbf{38.9})} & 34.33\scriptsize{(\textbf{47.07})} &  37.84\scriptsize{(\textbf{49.76})}         & \textbf{16.14}\scriptsize{(\textbf{20.31})} & \textbf{16.99}\scriptsize{(\textbf{23.41})} &  15.54\scriptsize{(\textbf{24.19})} \\
URE-GA-U & \textbf{34.59}\scriptsize{(36.39)} & \textbf{45.71}\scriptsize{(44.85)} &  \textbf{45.97}\scriptsize{(47.97)}     & 7.59\scriptsize{(10.06)} & 8.42\scriptsize{(11.52)} &   8.53\scriptsize{(12.75)} \\
URE-GA-R & 28.7\scriptsize{(30.94)} & 42.73\scriptsize{(43.34)} &  44.73\scriptsize{(47.36)}      & 5.24\scriptsize{(5.46)} & 6.77\scriptsize{(6.92)} &     5.0\scriptsize{(5.55)} \\
SCL-NL & 33.8\scriptsize{(37.81)} & 40.67\scriptsize{(42.58)} &   43.39\scriptsize{(45.2)}        & 7.58\scriptsize{(8.53)} & 6.77\scriptsize{(6.92)} &     5.0\scriptsize{(5.55)} \\
SCL-EXP & \textbf{34.59}\scriptsize{(36.96)} & 40.89\scriptsize{(42.99)} &    44.4\scriptsize{(47.9)}      & 7.55\scriptsize{(8.11)} & 7.42\scriptsize{(8.39)} &     8.0\scriptsize{(9.31)} \\
L-W & 28.04\scriptsize{(34.55)} & 34.96\scriptsize{(41.83)} &  39.05\scriptsize{(47.46)}          & 7.08\scriptsize{(8.74)} & 8.06\scriptsize{(8.76)} &   8.03\scriptsize{(10.18)} \\
L-UW & 30.63\scriptsize{(35.13)} & 38.05\scriptsize{(43.32)} &  39.49\scriptsize{(45.82)}         & 7.36\scriptsize{(8.71)} & 7.03\scriptsize{(8.55)} &   7.86\scriptsize{(10.11)} \\
PC-sigmoid & 24.38\scriptsize{(35.88)} & 25.63\scriptsize{(39.82)} &  33.89\scriptsize{(43.75)}                           & 9.27\scriptsize{(14.26)} & 11.91\scriptsize{(16.07)} &  \textbf{17.68}\scriptsize{(14.13)} \\
\bottomrule
\end{tabular}
\end{small}
}
\end{table}

==> Tables/name.tex <==
\begin{table}[ht]
\centering
\caption{}
% \vskip 0.15in
\label{tab:hard}
\resizebox{1\linewidth}{!}{%
% \scalebox{0.6}{
\begin{tabular}{lcccccccccccccccc}
\toprule
% & \multicolumn{2}{c}{CLCIFAR10} & & \multicolumn{2}{c}{CLCIFAR20} & & \multicolumn{2}{c}{CLMIN10} & & \multicolumn{2}{c}{CLMIN20} & & \multicolumn{2}{c}{Avg.} \\
& ResNet18 && ResNet34 && ResNet50 && DenseNet121 \\
% \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12} \cmidrule{14-15}
% & ResNet18 & ResNet34 & & ResNet18 & ResNet34 & & ResNet18 & ResNet34 & & ResNet18 & ResNet34 & & ResNet18 & ResNet34 \\
\midrule
scl-nl & 1.42 & & 1.63 && 1.19 && 1.36
fwd-r & 3.44 && 1.51 && 3.1 && 4.21
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/robust-loss-benchmark.tex <==
\begin{table}[ht]
\centering
\caption{Standard benchmark results on CLCIFAR and uniform-CIFAR datasets for the robust loss method. Mean accuracy ($\pm$ standard deviation) on the testing dataset from four trials with different random seeds. Highest accuracy in each column is highlighted in bold.} \label{tab:rob-loss}
% \vskip 0.15in
\resizebox{\columnwidth}{!}{%
\begin{small}
\begin{tabular}{lcccccccc}
\toprule
         & \multicolumn{2}{c}{uniform-CIFAR10} & \multicolumn{2}{c}{CLCIFAR10} & \multicolumn{2}{c}{uniform-CIFAR20} & \multicolumn{2}{c}{CLCIFAR20} \\ \midrule
methods  & valid\_acc     & valid\_acc (ES)    & valid\_acc  & valid\_acc (ES) & valid\_acc     & valid\_acc (ES)    & valid\_acc  & valid\_acc (ES) \\ \midrule
CCE & 46.57\scriptsize{$\pm$1.75} & 49.51\scriptsize{$\pm$0.73} & 16.18\scriptsize{$\pm$2.97} & 20.18\scriptsize{$\pm$3.39} & 12.54\scriptsize{$\pm$0.40} & 14.62\scriptsize{$\pm$1.29} & 5.07\scriptsize{$\pm$0.05} & 5.41\scriptsize{$\pm$0.30} \\
MAE & 57.37\scriptsize{$\pm$0.48} & 58.50\scriptsize{$\pm$0.97} & 16.30\scriptsize{$\pm$2.27} & 19.44\scriptsize{$\pm$4.41} & 16.72\scriptsize{$\pm$1.52} & 17.63\scriptsize{$\pm$1.63} & 5.11\scriptsize{$\pm$0.11} & 5.87\scriptsize{$\pm$0.26} \\
WMAE & - & - & 13.01\scriptsize{$\pm$1.89} & 15.51\scriptsize{$\pm$0.75} & - & - & 5.31\scriptsize{$\pm$0.27} & 6.65\scriptsize{$\pm$0.65} \\
GCE & 58.10\scriptsize{$\pm$1.54} & 59.44\scriptsize{$\pm$2.30} & 14.31\scriptsize{$\pm$1.44} & 18.97\scriptsize{$\pm$2.16} & 15.86\scriptsize{$\pm$1.93} & 17.09\scriptsize{$\pm$1.19} & 5.21\scriptsize{$\pm$0.29} & 5.76\scriptsize{$\pm$0.32} \\
SL & 41.13\scriptsize{$\pm$1.64} & 42.64\scriptsize{$\pm$0.11} & 16.45\scriptsize{$\pm$2.80} & 19.28\scriptsize{$\pm$3.16} & 13.60\scriptsize{$\pm$0.55} & 15.70\scriptsize{$\pm$1.23} & 5.44\scriptsize{$\pm$0.29} & 6.59\scriptsize{$\pm$0.43} \\
\bottomrule
\end{tabular}%
\end{small}
}
\end{table}

==> Tables/standard-benchmark.tex <==
\begin{table}[t]
\centering
\caption{Standard benchmark results on CLCIFAR and uniform-CIFAR datasets. Mean accuracy ($\pm$ standard deviation) on the testing dataset from four trials with different random seeds. Highest accuracy in each column is highlighted in bold.}
\label{tab:exp-1}
%vskip 0.05in
\resizebox{\columnwidth}{!}{%
\begin{small}
\begin{tabular}{lcccccccc}
\toprule
         & \multicolumn{2}{c}{uniform-CIFAR10} & \multicolumn{2}{c}{CLCIFAR10} & \multicolumn{2}{c}{uniform-CIFAR20} & \multicolumn{2}{c}{CLCIFAR20} \\ \midrule
methods  & valid\_acc     & valid\_acc (ES)    & valid\_acc  & valid\_acc (ES) & valid\_acc     & valid\_acc (ES)    & valid\_acc  & valid\_acc (ES) \\ \midrule
FWD-U     & \textbf{69.17\scriptsize{$\pm$1.22}}     & \textbf{69.79\scriptsize{$\pm$1.01}}         & 34.09\scriptsize{$\pm$1.16} & 36.83\scriptsize{$\pm$1.17}     & \textbf{20.24\scriptsize{$\pm$0.52}}     & 20.62\scriptsize{$\pm$0.49}         & 7.47\scriptsize{$\pm$0.37}  & 8.27\scriptsize{$\pm$0.77}      \\
FWD-R     & 68.89\scriptsize{$\pm$1.32}\footnotemark     & 69.32\scriptsize{$\pm$1.04}         & 28.88\scriptsize{$\pm$0.65} & \textbf{38.9\scriptsize{$\pm$1.57}}     & 19.98\scriptsize{$\pm$0.68}     & 20.71\scriptsize{$\pm$0.57}         & \textbf{16.14\scriptsize{$\pm$1.11}}  & \textbf{20.31\scriptsize{$\pm$0.25}}      \\
URE-GA-U     & 54.62\scriptsize{$\pm$0.6}     & 54.94\scriptsize{$\pm$1.34}         & \textbf{34.59\scriptsize{$\pm$0.76}} & 36.39\scriptsize{$\pm$0.67}     & 15.41\scriptsize{$\pm$0.97}     & 16.59\scriptsize{$\pm$0.61}         & 7.59\scriptsize{$\pm$0.36}  & 10.06\scriptsize{$\pm$0.72}      \\
URE-GA-R     & 53.29\scriptsize{$\pm$0.62}     & 57.02\scriptsize{$\pm$1.63}         & 28.7\scriptsize{$\pm$1.39} & 30.94\scriptsize{$\pm$1.66}     & 14.86\scriptsize{$\pm$1.06}     & 17.32\scriptsize{$\pm$0.8}         & 5.24\scriptsize{$\pm$0.2}  & 5.46\scriptsize{$\pm$0.28}      \\
SCL-NL     & 67.15\scriptsize{$\pm$1.9}     & 68.64\scriptsize{$\pm$1.98}         & 33.8\scriptsize{$\pm$0.52} & 37.81\scriptsize{$\pm$2.12}     & 20.04\scriptsize{$\pm$0.48}     & 20.68\scriptsize{$\pm$0.46}         & 7.58\scriptsize{$\pm$0.66}  & 8.53\scriptsize{$\pm$0.29}      \\
SCL-EXP     & 64.86\scriptsize{$\pm$0.44}     & 65.4\scriptsize{$\pm$0.32}         & 34.59\scriptsize{$\pm$0.72} & 36.96\scriptsize{$\pm$0.18}     & 19.4\scriptsize{$\pm$0.76}     & \textbf{21.03\scriptsize{$\pm$0.64}}         & 7.55\scriptsize{$\pm$0.51}  & 8.11\scriptsize{$\pm$0.71}      \\
L-W     & 56.21\scriptsize{$\pm$0.54}     & 59.18\scriptsize{$\pm$0.46}         & 28.04\scriptsize{$\pm$0.38} & 34.55\scriptsize{$\pm$2.05}     & 14.35\scriptsize{$\pm$0.74}     & 19.11\scriptsize{$\pm$1.29}         & 7.08\scriptsize{$\pm$1.1}  & 8.74\scriptsize{$\pm$0.42}      \\
L-UW     & 60.88\scriptsize{$\pm$0.77}     & 62.43\scriptsize{$\pm$0.46}         & 30.63\scriptsize{$\pm$1.87} & 35.13\scriptsize{$\pm$1.56}     & 16.01\scriptsize{$\pm$0.89}     & 19.42\scriptsize{$\pm$0.42}         & 7.36\scriptsize{$\pm$0.33}  & 8.71\scriptsize{$\pm$0.31}      \\
PC-sigmoid     & 28.20\scriptsize{$\pm$0.58} & 39.29\scriptsize{$\pm$0.87} & 24.38\scriptsize{$\pm$2.18} & 35.88\scriptsize{$\pm$0.98}     & 9.72\scriptsize{$\pm$0.49} & 16.45\scriptsize{$\pm$0.64} & 9.27\scriptsize{$\pm$0.37}  & 14.26\scriptsize{$\pm$1.04}      \\
\midrule
% CCE & 46.57\scriptsize{$\pm$1.75} & 49.51\scriptsize{$\pm$0.73} & 16.18\scriptsize{$\pm$2.97} & 20.18\scriptsize{$\pm$3.39} & 12.54\scriptsize{$\pm$0.40} & 14.62\scriptsize{$\pm$1.29} & 5.07\scriptsize{$\pm$0.05} & 5.41\scriptsize{$\pm$0.30} \\
MAE & 57.37\scriptsize{$\pm$0.48} & 58.50\scriptsize{$\pm$0.97} & 16.30\scriptsize{$\pm$2.27} & 19.44\scriptsize{$\pm$4.41} & 16.72\scriptsize{$\pm$1.52} & 17.63\scriptsize{$\pm$1.63} & 5.11\scriptsize{$\pm$0.11} & 5.87\scriptsize{$\pm$0.26} \\
\bottomrule
\toprule
& \multicolumn{4}{c}{\color{blue} CIFAR10} & \multicolumn{4}{c}{\color{blue}CIFAR20} \\
& \multicolumn{2}{c}{\color{blue}valid\_acc} & \multicolumn{2}{c}{\color{blue}valid\_acc(ES)} & \multicolumn{2}{c}{\color{blue}valid\_acc} & \multicolumn{2}{c}{\color{blue}valid\_acc(ES)} \\
\midrule
\color{blue} standard supervision & \multicolumn{2}{c}{\color{blue}82.70\scriptsize{$\pm$0.66}} & \multicolumn{2}{c}{\color{blue}82.80\scriptsize{$\pm$0.28}} & \multicolumn{2}{c}{\color{blue}63.23\scriptsize{$\pm$0.25}} & \multicolumn{2}{c}{\color{blue}63.80\scriptsize{$\pm$0.49}} \\
% GCE & 58.10\scriptsize{$\pm$1.54} & 59.44\scriptsize{$\pm$2.30} & 14.31\scriptsize{$\pm$1.44} & 18.97\scriptsize{$\pm$2.16} & 15.86\scriptsize{$\pm$1.93} & 17.09\scriptsize{$\pm$1.19} & 5.21\scriptsize{$\pm$0.29} & 5.76\scriptsize{$\pm$0.32} \\
% SL & 41.13\scriptsize{$\pm$1.64} & 42.64\scriptsize{$\pm$0.11} & 16.45\scriptsize{$\pm$2.80} & 19.28\scriptsize{$\pm$3.16} & 13.60\scriptsize{$\pm$0.55} & 15.70\scriptsize{$\pm$1.23} & 5.44\scriptsize{$\pm$0.29} & 6.59\scriptsize{$\pm$0.43} \\
\bottomrule
\end{tabular}%
\end{small}
}
\end{table}

\footnotetext{Note that FWD-R and URE-GA-R assume the empirical transition matrix $T_e$ to be provided. The empirical transition matrix is computed from the labels in the training set, so it is slightly different from a uniform transition matrix $T_u$ in the uniform-CIFAR datasets. As a result, the performances of FWD-R and URE-GA-R do not exactly match those of FWD-U and URE-GA-U, respectively, in the uniform-CIFAR datasets.}

==> Tables/strategies.tex <==
\begin{table}[ht]
\centering
\caption{Overview of strategies included in the \texttt{libcll} toolkit.}
% \vskip 0.15in
\label{tab:strategies}
\setlength{\tabcolsep}{10pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.5} % Default value: 1
\resizebox{1\linewidth}{!}{%
\scalebox{0.50}{
\begin{tabular}{l|c|l}
\hline
Strategy & Type & Description \\
\hline
\multirow{2}{4em}{SCL~\cite{scl2020}} & NL & Surrogate Complementary Loss with negative log loss. \\
& EXP & Surrogate Complementary Loss with exponential loss. \\
\hline
\multirow{4}{4em}{URE~\cite{ishida2019complementarylabel}} & NN & Unbiased risk estimator with uniform transition matrix. \\
& GA & Gradient Ascent applied to the unbiased risk estimator with uniform transition matrix. \\
& TNN & Unbiased risk estimator with true transition matrix. \\
& TGA & Gradient Ascent applied to the unbiased risk estimator with true transition matrix. \\
\hline
DM~\cite{gao2021discriminative} & - & Discriminative Models with Weighted Loss. \\
\hline
FWD~\cite{fwd2018} & - & Forward Correction. \\
\hline
\multirow{3}{4em}{CPE~\cite{cpe2023}} & I & Complementary Probability Estimates. \\
& F & Complementary Probability Estimates with true transition matrix. \\
& T & Complementary Probability Estimates with trainable transition matrix. \\
\hline
\multirow{3}{4em}{MCL~\cite{mcl2020}} & MAE & Multiple Complementary Loss with mean absolute error. \\
& EXP & Multiple Complementary Loss with exponential loss. \\
& LOG & Multiple Complementary Loss with negative log loss. \\
\bottomrule
\end{tabular}%
}}
\end{table}

==> Tables/test.tex <==
\begin{table}[ht]
\centering
\caption{}
% \vskip 0.15in
\resizebox{1\linewidth}{!}{
\begin{tabular}{lccccccccccccccccccccc}
\toprule
& \multicolumn{4}{c}{CLCIFAR10} & & \multicolumn{4}{c}{CLCIFAR20} & & \multicolumn{4}{c}{CLMIN10} & & \multicolumn{4}{c}{CLMIN20} \\
\cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-15} \cmidrule{17-20}
& ResNet18 & ResNet34 & ResNet50 & DenseNet121 & & ResNet18 & ResNet34 & ResNet50 & DenseNet121 & & ResNet18 & ResNet34 & ResNet50 & DenseNet121 & & ResNet18 & ResNet34 & ResNet50 & DenseNet121 \\
\midrule
scl-nl & 34.77 & 25.13 & 24.55 & 31.42 & & 8.02 & 5.62 & 7.45 & 7.98 & & 21.8 &  12.60 & 10.40 & 11.40 & & 6.17 & 5.00 & 3.60 & 5.10\\
fwd-r & 38.12 & 27.60 & 26.06 & 27.09 & & 20.27 & 12.21 & 13.78 & 14.26 & & 30.15 &  15.20 & 21.00 & 15.80 & & 10.6 & 5.80 & 6.80 & 6.50\\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/validation.tex <==
\begin{table}[t]
\centering
\caption{The testing accuracy of models evaluated with URE and SCEL.} %on a complementary validation set.}
\label{tab:valid}
\vskip 0.05in
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc|cccc|cccc|cccc}
\toprule
           & \multicolumn{4}{c}{uniform-cifar10}                                                                          & \multicolumn{4}{c}{clcifar10}                                                                                & \multicolumn{4}{c}{uniform-cifar20}                                                                          & \multicolumn{4}{c}{clcifar20}                                                                                \\
           \midrule
           & \multicolumn{1}{l}{URE} & \multicolumn{1}{l}{SCEL} & \multicolumn{1}{l}{valid acc} & \multicolumn{1}{l}{gap ($\downarrow$)} & \multicolumn{1}{l}{URE} & \multicolumn{1}{l}{SCEL} & \multicolumn{1}{l}{valid acc} & \multicolumn{1}{l}{gap ($\downarrow$)} & \multicolumn{1}{l}{URE} & \multicolumn{1}{l}{SCEL} & \multicolumn{1}{l}{valid acc} & \multicolumn{1}{l}{gap ($\downarrow$)} & \multicolumn{1}{l}{URE} & \multicolumn{1}{l}{SCEL} & \multicolumn{1}{l}{valid acc} & \multicolumn{1}{l}{gap ($\downarrow$)} \\
           \midrule
FWD-U      & 22.36                   & 45.63                    & 48.44                         & 2.81                    & 32.54                   & 33.02                    & 34.09                         & 1.07                    & 16.02                   & 16.02                    & 17.4                          & 1.38                    & 7.33                    & 7.33                     & 7.47                          & 0.14                    \\
FWD-R      & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}    & \multicolumn{1}{l}{-}         & \multicolumn{1}{l}{-}   & 28.88                   & 19.13                    & 28.88                         & 0                       & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}    & \multicolumn{1}{l}{-}         & \multicolumn{1}{l}{-}   & 10.74                   & 9.8                      & 16.14                         & 5.4                     \\
URE-GA-U   & 39.24                   & 39.24                    & 39.55                         & 0.31                    & 31.34                   & 34.59                    & 34.59                         & 0                       & 13.12                   & 12.64                    & 13.52                         & 0.4                     & 7.28                    & 7.85                     & 7.59                          & -0.26                   \\
URE-GA-R   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}    & \multicolumn{1}{l}{-}         & \multicolumn{1}{l}{-}   & 26.61                   & 28.18                    & 28.7                          & 0.52                    & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}    & \multicolumn{1}{l}{-}         & \multicolumn{1}{l}{-}   & 5.2                     & 5.36                     & 5.24                          & -0.12                   \\
SCL-NL     & 22.83                   & 36.44                    & 48.2                          & 11.76                   & 32.49                   & 33.32                    & 33.8                          & 0.48                    & 14.16                   & 16.55                    & 16.55                         & 0                       & 7.12                    & 6.5                      & 7.58                          & 0.46                    \\
SCL-EXP    & 22.72                   & 22.72                    & 46.79                         & 24.07                   & 33.15                   & 31.26                    & 34.59                         & 1.44                    & 14.23                   & 14.16                    & 16.18                         & 1.95                    & 6.85                    & 6.53                     & 7.55                          & 0.7                     \\
L-W        & 10.38                   & 11.03                    & 27.02                         & 15.99                   & 20.71                   & 20.71                    & 28.04                         & 7.33                    & 7.37                    & 9.66                     & 10.39                         & 0.73                    & 5.77                    & 6.03                     & 7.08                          & 1.05                    \\
L-UW       & 9.93                    & 9.93                     & 31.3                          & 21.37                   & 22.97                   & 22.97                    & 30.63                         & 7.66                    & 7.68                    & 7.68                     & 12.33                         & 4.65                    & 5.9                     & 5.9                      & 7.36                          & 1.46                    \\
PC-sigmoid & 16.07                   & 15.62                    & 18.97                         & 2.9                     & 14.98                   & 15.43                    & 24.38                         & 8.95                    & 7.38                    & 7.38                     & 7.67                          & 0.29                    & 7.04                    & 8.63                     & 9.27                          & 0.64                   \\
\bottomrule
\end{tabular}%
}
% \vskip -0.1in
\end{table}
